Towards Agentic Recommender Systems in the Era of Multimodal Large Language Models

Recent breakthroughs in Large Language Models (LLMs) have led to the emergence of agentic AI systems that extend beyond the capabilities of standalone models. By empowering LLMs to perceive external environments, integrate multimodal information, and interact with various tools, these agentic systems exhibit greater autonomy and adaptability across complex tasks. This evolution brings new opportunities to recommender systems (RS): LLM-based Agentic RS (LLM-ARS) can offer more interactive, context-aware, and proactive recommendations, potentially reshaping the user experience and broadening the application scope of RS. Despite promising early results, fundamental challenges remain, including how to effectively incorporate external knowledge, balance autonomy with controllability, and evaluate performance in dynamic, multimodal settings. In this perspective paper, we first present a systematic analysis of LLM-ARS: (1) clarifying core concepts and architectures; (2) highlighting how agentic capabilities -- such as planning, memory, and multimodal reasoning -- can enhance recommendation quality; and (3) outlining key research questions in areas such as safety, efficiency, and lifelong personalization. We also discuss open problems and future directions, arguing that LLM-ARS will drive the next wave of RS innovation. Ultimately, we foresee a paradigm shift toward intelligent, autonomous, and collaborative recommendation experiences that more closely align with users' evolving needs and complex decision-making processes.

==> 3_Related_Survey.tex <==

\section{Related Surveys}

LLM-based agents in general domains have been widely discussed and surveyed \cite{GuoCWCPCW024,WangMFZYZCTCLZWW24}. Different from these surveys, this survey focuses on the design and application of LLM-based agents specifically for the recommender systems domain. In the recommender systems domain, 
% there have been several surveys or literature reviews on the general application of LLMs in recommender systems \cite{} .
multiple reviews have been conducted on the intersection of LLMs and RecSys. 
Liu \textit{et al.} \cite{survey2} delves into the training strategies and learning objectives of language modeling paradigm adaptations for recommenders, while Wu \textit{et al.} \cite{survey3} provides insights from both discriminative and generative viewpoints on Language Model-based Recommender Systems (LLM4Rec). Lin \textit{et al.} \cite{survey1} introduces two orthogonal perspectives: where and how to adapt LLMs in recommender systems. Fan \textit{et al.} \cite{survey4} offers an overview of LLMs for recommender systems, concentrating on paradigms such as pre-training, fine-tuning, and prompting. Lin \textit{et al.} \cite{survey5} summarizes the current progress in generative recommendations, organizing them across various recommendation tasks.
% All Roads Lead to Rome: Unveiling the Trajectory of Recommender Systems Across the LLM Era
Bo \textit{et al.} \cite{Bochen} explores the evolution of recommender systems, mainly including the list-wise and conversational recommendation systems, highlighting the transformation from static recommendations to LLM agent RSs. 

==> tables/agent_table.tex <==
% \begin{table*}[t!]
% \small
% \centering
% \begin{tabular}{cccccc}
% \toprule
% \textbf{Model} & \textbf{Objectives} & \textbf{Single-type Agents} & \textbf{Multi-type Agents}  & \textbf{Diverse Rec. Scenarios} & \textbf{Open-source} \\
% \midrule
% RecAgent~\cite{wang2023recagent} & User Simulation & \Checkmark &  &  & \Checkmark \\
% Agent4Rec~\cite{agent4rec} & User  Simulation & \Checkmark &  &  &  \Checkmark \\
% LLM-Ins~\cite{Feiran24} & User  Simulation & \Checkmark &  &  &   \\
% PMG~\cite{ShenZ0ZX24} & User  Simulation & \Checkmark &  &  &  \Checkmark \\
% BiLLP~\cite{BiLLP24} & User  Simulation & \Checkmark &  &  &  \Checkmark \\
% BASES~\cite{BASES24} & User  Simulation & \Checkmark &  &  &   \\
% USimAgent~\cite{Erhan24} & User  Simulation & \Checkmark &  &  &   \\
% AgentCF~\cite{AgentCF} & U-I Inter Simulation & & \Checkmark &  &  \\
% WebAgent~\cite{cai2024large} & U-I Inter Simulation & & \Checkmark & \Checkmark &  \Checkmark\\
% \midrule
% RAH~\cite{Yubo23} & Recommender &  & \Checkmark &  &  \\
% RecMind~\cite{wang2023recmind}  & Recommender & \Checkmark &  & \Checkmark &  \\
% InteRecAgent~\cite{InteRecAgent}  & Recommender & \Checkmark &  &  & \\
% MACRec~\cite{Zhefan24} & Recommender  & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\
% \bottomrule
% \end{tabular}
% \vspace{0.5cm} % Adjust the value as needed
% \caption{Comparison among \textbf{Personalized Agent for RecSys with Foundation Models}. Note that \textsl{Single-type Agents} indicate all agents serve the same role (e.g., users), while \textsl{Multi-type Agents} refer to agents having multiple roles and capabilities (e.g., managers, reflectors).}
% \label{tab:agent_paper}
% \end{table*}


\begin{table*}[t!]
\small
% \large
% \scriptsize 
\centering
% \setlength{\tabcolsep}{4pt} 
% \renewcommand{\arraystretch}{0.95} 
\begin{tabular}{cccccc}
\toprule
\textbf{Model} & \textbf{Objectives} & \textbf{Single-type Agents} & \textbf{Multi-type Agents} & \textbf{Diverse Rec. Scenarios} & \textbf{Open-source} \\
\midrule
RecAgent~\cite{wang2023recagent} & User Simulation & \Checkmark &  &  & \Checkmark \\
Agent4Rec~\cite{agent4rec} & User Simulation & \Checkmark &  &  & \Checkmark \\
LLM-Ins~\cite{Feiran24} & User Simulation & \Checkmark &  &  &  \\
PMG~\cite{ShenZ0ZX24} & User Simulation & \Checkmark &  &  & \Checkmark \\
BiLLP~\cite{Shi0ZGLZWF24} & User Simulation & \Checkmark &  &  & \Checkmark \\
BASES~\cite{BASES24} & User Simulation & \Checkmark &  &  &  \\
USimAgent~\cite{Erhan24} & User Simulation & \Checkmark &  &  &  \\
AgentCF~\cite{AgentCF} & U-I Inter Simulation &  & \Checkmark &  &  \\
WebAgent~\cite{Hongru} & U-I Inter Simulation &  & \Checkmark & \Checkmark & \Checkmark \\
\midrule
RAH~\cite{Yubo23} & Recommender &  & \Checkmark &  &  \\
RecMind~\cite{wang2023recmind} & Recommender & \Checkmark &  & \Checkmark &  \\
InteRecAgent~\cite{InteRecAgent} & Recommender & \Checkmark &  &  &  \\
MACRec~\cite{Zhefan24} & Recommender & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\
\bottomrule
\end{tabular}
\caption{Comparison among \textbf{Personalized Agent for RecSys with Foundation Models}. Note that \textsl{Single-type Agents} indicate all agents serve the same role (e.g., users), while \textsl{Multi-type Agents} refer to agents having multiple roles and capabilities (e.g., managers, reflectors).}
\label{tab:agent_paper}
\end{table*}


==> tables/overview.tex <==
% \begin{figure*}[t!]
% \centering
% \large
% \begin{forest}
% for tree={   
% font=\small, 
% % style of nodes in the tree
% draw=myblue, semithick, rounded corners,
%        minimum height = 1.5ex,
%         minimum width = 2em,
% % style of tree (edges, distances, direction)
%     anchor = west,
%      grow = east,
% forked edge,        % for forked edge
%     s sep = 0.8mm,    % "sibling" distance
%     l sep = 3.5mm,    % "level" distance
%  fork sep = 2mm,    % distance from parent to branching point
%            }
% [The Classification of AgenticRS, rotate=90, anchor=center
%     [\S \ref{sec:agent_perspective} Agent Perspective, text width=1.2cm
%         [\S \ref{sec:single_agent} Single Agent Framework for RS, text width=2.5cm
%             [{}, text width=9.3cm, fill=lightblue]
%         ]
%         [\S \ref{sec:multi_agent} Multi-Agent Framework for RS, text width=2.5cm
%             [{}, text width=9.3cm, fill=lightblue]
%         ]
%         [\S \ref{sec:human_agent} Human-LLM agent Collaboration for RS, text width=2.5cm
%             [{}, text width=9.3cm, fill=lightblue]
%         ]
%         [\S \ref{sec:evaluation} Evaluation, text width=2.5cm
%             [{}, text width=9.3cm, fill=lightblue]
%         ]
%     ]
% ]
% \end{forest}
% \caption{The Classification of Agentic Recommender Systems.}
% \label{fig:task_overview}
% \end{figure*}

\begin{figure*}[t!]
\centering
\large
\begin{forest}
for tree={   
font=\small, 
% style of nodes in the tree
draw=myblue, semithick, rounded corners,
       minimum height = 1.5ex,
        minimum width = 2em,
% style of tree (edges, distances, direction)
    anchor = west,
     grow = east,
forked edge,        % for forked edge
    s sep = 0.8mm,    % "sibling" distance
    l sep = 3.5mm,    % "level" distance
 fork sep = 2mm,    % distance from parent to branching point
           }
[The Classification of AgenticRS, rotate=90, anchor=center
    [\S Preliminary, text width=3cm
        [LLM-based Single Agent Systems, text width=3cm
            [{}, text width=9.3cm, fill=lightblue]
        ]
        [LLM-based Multi-agent Systems, text width=3cm
            [{}, text width=9.3cm, fill=lightblue]
        ]
        [The Memory Module, text width=3cm
            [{}, text width=9.3cm, fill=lightblue]
        ]
        [The Action Module, text width=3cm
            [{}, text width=9.3cm, fill=lightblue]
        ]
    ]
    [\S Analysis from Agent Perspective, text width=3cm
        % [Agent Architectures for RS, text width=3cm
        %     [{}, text width=9.3cm, fill=lightblue]
        % ]
        [Planning and Reasoning in Agentic RS, text width=3cm
            [{MACRec~\cite{wang2024macrec}, ToolRec~\cite{zhao2024let}, iALP~\cite{wang2025large}, ChatCRS~\cite{li2024incorporating}, 
            MACRS~\cite{fang2024multi}, KGLA~\cite{guo2024knowledge}, RDRec~\cite{wang2024rdrec}, MemoCRS~\cite{xi2024memocrs}, 
            PC-CRS~\cite{qin2024beyond}, LANE~\cite{zhao2024lane}, CoRAL~\cite{wu2024coral}}, text width=9.3cm, fill=lightblue]
        ]
        [Agent Self-Improvement, text width=3cm
            [{iALP~\cite{wang2025large}, LEA~\cite{wang2024reinforcement}, AgentRec~\cite{park2025agentrec}, 
            LANE~\cite{zhao2024lane}, CoRAL~\cite{wu2024coral}}, text width=9.3cm, fill=lightblue]
        ]
        [LLM-Agent Roleplaying in User Modeling, text width=3cm
            [{AgentCF~\cite{zhang2024agentcf}, \citet{zhang2024llm}, \citet{wang2024user}, CSHI~\cite{zhu2024llm}, 
            LLM-RSE~\cite{corecco2024llm}, PEPPER~\cite{kim2024stop}, Lusifer~\cite{ebrat2024lusifer}}, text width=9.3cm, fill=lightblue]
        ]
        [Interaction Between Agents and Users, text width=3cm
            [{AgentCF~\cite{zhang2024agentcf}, InteRecAgent~\cite{huang2023recommender}, ELMRec~\cite{wang2024enhancing}, 
            MACRec~\cite{wang2024macrec}, MACRS~\cite{fang2024multi}, PEPPER~\cite{kim2024stop}}, text width=9.3cm, fill=lightblue]
        ]
    ]
    [\S Analysis from RS Perspective, text width=3cm
        [Single Agent Framework for RS, text width=3cm
            [{RecAgent \cite{agent4rec},  }, text width=9.3cm, fill=lightblue]
        ]
        [Multi-Agent Framework for RS, text width=3cm
            [{}, text width=9.3cm, fill=lightblue]
        ]
        [Human-LLM Agent Collaboration for RS, text width=3cm
            [{}, text width=9.3cm, fill=lightblue]
        ]
    ]
    [\S Open Problems and Opportunities, text width=3cm
        [Efficiency, text width=3cm
            [{}, text width=9.3cm, fill=lightblue]
        ]
        [Benchmarking, text width=3cm
            [{}, text width=9.3cm, fill=lightblue]
        ]
        [Hallucination, text width=3cm
            [{}, text width=9.3cm, fill=lightblue]
        ]
    ]
]
\end{forest}
\caption{The Classification of Agentic Recommender Systems.}
\label{fig:task_overview}
\end{figure*}

